Corruption-Robust Offline Reinforcement Learning

We study the adversarial robustness in offline reinforcement learning. Given a batch dataset consisting of tuples $(s, a, r, s')$, an adversary is allowed to arbitrarily modify $\epsilon$ fraction of the tuples. From the corrupted dataset the learner aims to robustly identify a near-optimal policy. We first show that a worst-case $\Omega(d\epsilon)$ optimality gap is unavoidable in linear MDP of dimension $d$, even if the adversary only corrupts the reward element in a tuple. This contrasts with dimension-free results in robust supervised learning and best-known lower-bound in the online RL setting with corruption. Next, we propose robust variants of the Least-Square Value Iteration (LSVI) algorithm utilizing robust supervised learning oracles, which achieve near-matching performances in cases both with and without full data coverage. The algorithm requires the knowledge of $\epsilon$ to design the pessimism bonus in the no-coverage case. Surprisingly, in this case, the knowledge of $\epsilon$ is necessary, as we show that being adaptive to unknown $\epsilon$ is impossible.This again contrasts with recent results on corruption-robust online RL and implies that robust offline RL is a strictly harder problem.

==> Corruption-Robust Offline Reinforcement Learning/algorithm.tex <==


%\subsection{Earlier notes for tabular MDP}
%
%Given the offline dataset $\{s_i, a_i, r_i, s_i'\}_{i=1}^N$ which potentially is corrupted in both transition and rewards, and the upper bound on the corruption level, i.e., $C \in \mathbb{N}^+$ is the upper bound on the total number of corrupted $(s,a,r,s')$ tuples. 
%
%Let us consider tabular MDP for now, and we should be able to extend it to linear MDP or Kernelized Nonlinear Regulator (KNR).  Let us use offline data to design the following reward bonus:
%\begin{align*}
%b(s,a) = \min \left\{ \frac{1}{1-\gamma}  \sqrt{ \frac{ \ln(SA /\delta)  }{ N(s,a)} } + \frac{ C \ln(SA /\delta) }{N(s,a)},  \frac{1}{1-\gamma} \right\}, 
%\end{align*} where $N(s,a) = \sum_{i=1}^N \mathbf{1}\{(s,a) = (s_i,a_i)\}$.  \wen{the constant terms and log terms might be sloppy here for now..Also I think the bonus here might need to scale with an additional $\sqrt{S}$}
%
%Let us fit a reward estimator and transition estimator as follows:
%\begin{align*}
%&\widehat{P}(s' | s,a) = \frac{ \sum_{i=1}^N \mathbf{1}\{(s_i,a_i,s_i') = (s,a,s)\} }{N(s,a)}, \quad  \widehat{r}(s,a) = \sum_{i=1}^{N} r_i \mathbf{1}\{ (s_i,a_i) = (s,a) \} / N.
%\end{align*}  \wen{need to deal with the $(s,a)$ pair that have zero visit counts..}
%
%Let us consider the following pessimism-based model-based algorithm:
%\begin{align*}
%\widehat{\pi} = \text{Policy Iteration}\left( \widehat{P}, \widehat{r} - b \right).
%\end{align*}
%
%Below is the proof sketch. We first prove that the bonus is a valid to provide pessimism for all policy $\pi$ \wen{this is where the additional $\sqrt{S}$ maybe needed in bonus}:  
%\begin{align*}
%\forall \pi: \;  \widehat{V}^{\pi} \leq V^{\pi},
%\end{align*} where $\widehat{V}^{\pi}$ is the value of $\pi$ under $(\widehat{P}, \widehat{r} - b)$.
%Consider a benchmark policy $\widetilde{\pi}$ (not necessarily has to be $\pi^\star$, as $\pi^\star$ might be covered by the offline data at all)
%\begin{align*}
%&V^{\widetilde\pi} - V^{\widehat\pi} \leq V^{\widetilde\pi} - \widehat{V}^{\widehat\pi} \leq V^{\widetilde\pi} - \widehat{V}^{\widetilde\pi} \\
%& =\frac{1}{1-\gamma} \mathbb{E}_{s,a\sim \widetilde\pi} \left[  b(s,a) + \left\lvert \mathbb{E}_{s'\sim \widehat{P}_{s,a}} \widehat{V}^{\widetilde\pi}(s') - \mathbb{E}_{s'\sim P_{s,a}} \widehat{V}^{\widetilde\pi}(s')    \right\rvert\right] \\
%& \leq  \frac{2}{1-\gamma} \mathbb{E}_{s,a\sim \widetilde\pi} \left[  b(s,a) \right].
%\end{align*} Rearrange terms, we get:
%\begin{align*}
%V^{\widehat\pi} \geq \max_{\widetilde\pi} \left( V^{\widetilde\pi} - \frac{2}{1-\gamma} \mathbb{E}_{s,a\sim \widetilde\pi} b(s,a) \right).
%\end{align*} Intuitively, the $\widetilde\pi$ here should be the policy that achieves the highest total reward while being constrained inside the offline data's coverage (i.e., does not have high expected total reward bonus). For special case where the offline data only provides coverage under $\pi^\star$, i.e., $\sup_{s,a} d^{\pi^\star}(s,a) / \rho(s,a) \leq C$, we should work out the detailed bound.  Note that this assumption is significantly weaker than the uniform coverage assumption. 
%
%\subsection{Algorithms for Unknown Corruption Level}
%
%\wen{no idea yet...maybe the multi-layer sub-sampling algorithm will just work, even though we will not be able to tolerate constant corruption level, which might be ok for now...}
%
%Let us consider the following simplified setting: we assume that there is either no corruption at all, or there are at most $C$ many corrupted tuples.  Can we design an algorithm that automatically achieves good performance under these two settings even without knowing which setting it falls into. This should be the first step towards the unknown $C$. 




==> Corruption-Robust Offline Reinforcement Learning/def.tex <==
\newcommand{\M}{\mathcal{M}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\RR}{\mathcal{R}}
\newcommand{\bv}[1]{\mathbf{#1}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\poly}{\text{poly}}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\Var}{\operatorname{Var}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{assumption}{Assumption}[section]
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem*{lemma*}{Lemma}
\newtheorem{proposition}{Proposition}[section]

\newcommand{\eqnref}[1]{Eqn.~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\wen}[1]{{\color{blue}[\textbf{WS:} #1]}}
\newcommand{\XZ}[1]{{\color{red}[\textbf{XZ:} #1]}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\Kcal}{\mathcal{K}}
\renewcommand{\S}{\mathcal{S}}
\renewcommand\ind[1]{\ensuremath{\mathds{1}\left[#1\right]}}
\renewcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\interior}[1]{%
	{\kern0pt#1}^{\mathrm{o}}%
}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\newcommand\gwp{\overset{\mathclap{\normalfont\mbox{\small{w.p. 1-p}}}}{\geq}}

\newcommand{\1}{\mathbbm{1}}

\newcommand{\Scal}{\mathcal{S}}
\newcommand{\oper}{\mbox{op}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\EE}{\ensuremath{\mathbb{E}}}
\newcommand{\sa}{(s,a)}
\newcommand{\wh}{\ensuremath{\widehat w}}
\newcommand{\sL}{\mathcal{L}}
\newcommand{\filter}{{\textsc{Filter}}}
\newcommand{\one}{\mathbf{1}}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

\newcommand{\Pb}{\mathbb{P}}
\newcommand{\Bb}{\mathbb{B}}
\newcommand{\subopt}{\mbox{SubOpt}}

==> algorithm.tex <==


%\subsection{Earlier notes for tabular MDP}
%
%Given the offline dataset $\{s_i, a_i, r_i, s_i'\}_{i=1}^N$ which potentially is corrupted in both transition and rewards, and the upper bound on the corruption level, i.e., $C \in \mathbb{N}^+$ is the upper bound on the total number of corrupted $(s,a,r,s')$ tuples. 
%
%Let us consider tabular MDP for now, and we should be able to extend it to linear MDP or Kernelized Nonlinear Regulator (KNR).  Let us use offline data to design the following reward bonus:
%\begin{align*}
%b(s,a) = \min \left\{ \frac{1}{1-\gamma}  \sqrt{ \frac{ \ln(SA /\delta)  }{ N(s,a)} } + \frac{ C \ln(SA /\delta) }{N(s,a)},  \frac{1}{1-\gamma} \right\}, 
%\end{align*} where $N(s,a) = \sum_{i=1}^N \mathbf{1}\{(s,a) = (s_i,a_i)\}$.  \wen{the constant terms and log terms might be sloppy here for now..Also I think the bonus here might need to scale with an additional $\sqrt{S}$}
%
%Let us fit a reward estimator and transition estimator as follows:
%\begin{align*}
%&\widehat{P}(s' | s,a) = \frac{ \sum_{i=1}^N \mathbf{1}\{(s_i,a_i,s_i') = (s,a,s)\} }{N(s,a)}, \quad  \widehat{r}(s,a) = \sum_{i=1}^{N} r_i \mathbf{1}\{ (s_i,a_i) = (s,a) \} / N.
%\end{align*}  \wen{need to deal with the $(s,a)$ pair that have zero visit counts..}
%
%Let us consider the following pessimism-based model-based algorithm:
%\begin{align*}
%\widehat{\pi} = \text{Policy Iteration}\left( \widehat{P}, \widehat{r} - b \right).
%\end{align*}
%
%Below is the proof sketch. We first prove that the bonus is a valid to provide pessimism for all policy $\pi$ \wen{this is where the additional $\sqrt{S}$ maybe needed in bonus}:  
%\begin{align*}
%\forall \pi: \;  \widehat{V}^{\pi} \leq V^{\pi},
%\end{align*} where $\widehat{V}^{\pi}$ is the value of $\pi$ under $(\widehat{P}, \widehat{r} - b)$.
%Consider a benchmark policy $\widetilde{\pi}$ (not necessarily has to be $\pi^\star$, as $\pi^\star$ might be covered by the offline data at all)
%\begin{align*}
%&V^{\widetilde\pi} - V^{\widehat\pi} \leq V^{\widetilde\pi} - \widehat{V}^{\widehat\pi} \leq V^{\widetilde\pi} - \widehat{V}^{\widetilde\pi} \\
%& =\frac{1}{1-\gamma} \mathbb{E}_{s,a\sim \widetilde\pi} \left[  b(s,a) + \left\lvert \mathbb{E}_{s'\sim \widehat{P}_{s,a}} \widehat{V}^{\widetilde\pi}(s') - \mathbb{E}_{s'\sim P_{s,a}} \widehat{V}^{\widetilde\pi}(s')    \right\rvert\right] \\
%& \leq  \frac{2}{1-\gamma} \mathbb{E}_{s,a\sim \widetilde\pi} \left[  b(s,a) \right].
%\end{align*} Rearrange terms, we get:
%\begin{align*}
%V^{\widehat\pi} \geq \max_{\widetilde\pi} \left( V^{\widetilde\pi} - \frac{2}{1-\gamma} \mathbb{E}_{s,a\sim \widetilde\pi} b(s,a) \right).
%\end{align*} Intuitively, the $\widetilde\pi$ here should be the policy that achieves the highest total reward while being constrained inside the offline data's coverage (i.e., does not have high expected total reward bonus). For special case where the offline data only provides coverage under $\pi^\star$, i.e., $\sup_{s,a} d^{\pi^\star}(s,a) / \rho(s,a) \leq C$, we should work out the detailed bound.  Note that this assumption is significantly weaker than the uniform coverage assumption. 
%
%\subsection{Algorithms for Unknown Corruption Level}
%
%\wen{no idea yet...maybe the multi-layer sub-sampling algorithm will just work, even though we will not be able to tolerate constant corruption level, which might be ok for now...}
%
%Let us consider the following simplified setting: we assume that there is either no corruption at all, or there are at most $C$ many corrupted tuples.  Can we design an algorithm that automatically achieves good performance under these two settings even without knowing which setting it falls into. This should be the first step towards the unknown $C$. 



